Human-Robot Commensality: Bite Timing Prediction for Robot-Assisted Feeding in Groups

We develop data-driven models to predict when a robot should feed during social dining scenarios. Being able to eat independently with friends and family is considered one of the most memorable and important activities for people with mobility limitations. While existing robotic systems for feeding people with mobility limitations focus on solitary dining, commensality, the act of eating together, is often the practice of choice. Sharing meals with others introduces the problem of socially appropriate bite timing for a robot, i.e. the appropriate timing for the robot to feed without disrupting the social dynamics of a shared meal. Our key insight is that bite timing strategies that take into account the delicate balance of social cues can lead to seamless interactions during robot-assisted feeding in a social dining scenario. We approach this problem by collecting a Human-Human Commensality Dataset (HHCD) containing 30 groups of three people eating together. We use this dataset to analyze human-human commensality behaviors and develop bite timing prediction models in social dining scenarios. We also transfer these models to human-robot commensality scenarios. Our user studies show that prediction improves when our algorithm uses multimodal social signaling cues between diners to model bite timing. The HHCD dataset, videos of user studies, and code are available at https://emprise.cs.cornell.edu/hrcom/

==> sections/2_related_work.tex <==
\section{Related Work}\label{sec:related_work}
% Robots have the potential to increase or prolong unassisted living for people with mobility impairments \cite{}. 
% Feeding in social scenarios requires implicitly or explicitly probing the user to feed, even when they might be in a conversation.
% Parallels can be drawn to interruptibility research on finding the most appropriate timing to probe a user.
% Research in probing users when they are busy is known as interruptibility, which has been extensively studied by the human-computer interaction and human-robot interaction communities. 
% Our work aims to use various social signals to learn a bite timing strategy for a robot that can feed a user in a social dining setting. % reword this
% Researchers have found that people performed best on a task if interruptions were mediated rather than timed immediately or on scheduled intervals \cite{mcfarlane2002comparison,czerwinski2000instant}.
% As sensors become more widespread and large amounts of data is easier to collect, machine-learning based approaches are becoming more accurate at predicting interruptibility by considering contextual and social factors \cite{pielot2017beyond, takemae2007estimating, banerjee2018effects, wu2021learning}.
% Capturing these natural social interactions in computational models are crucial to provide services without distracting users from the social ambiance. 
% Features such as gaze, speaking interactions, body pose have all been effective measures in learning social signals of humans \cite{wang2021multi, muller2018robust, park20123d, joo2019towards}.
% Joo et al.~\cite{joo2019towards} presented a framework to model social interactions by predicting whether a person is speaking or by predicting their body gestures while looking only at other conversational partners.
% Similarly, this work focuses on capturing social interactions from a set of diners to develop a bite timing strategy that can feed a target user on a robot.
% Using data of able-bodied humans eating together, we propose leveraging similar models on interruptibility on social features to learn when an ideal time a robot should interrupt a user to feed.
% Therefore, we use inspiration not only from robot-assisted feeding and interruptibility literature but also from social signals modeling research.

% Moreover, the objective is to predict user's bite intention in a social dining settings. 
% Our work connects social signal modeling research with robot-assisted feeding and HCI interruption area.

% \textbf{Robot-assisted Feeding Systems}
% Prior researchers have developed various robot-assisted feeding systems in various different forms \cite{candeias2018vision, higa2014vision, jardon2012functional, bhattacharjee2019towards, park2016towards, alqasemi2005wheelchair, bien2004integration, park2016towards}.
% These techniques are purely reactive which means users must order the robot to feed by pushing a button, saying a word, or using an interface.
% Most of these techniques are purely reactive, where the user must order the robot to feed using some form of an interface
% Recent work in social dining \cite{herlant2018algorithms} has attempted to learn when to feed using an HMM trained on a single user. Although the their system was evaluated in a dyadic robot-assisted feeding scenario, the model was trained only on the user's data and likely does not capture complex group social interactions.
% Bhattacharjee et al.~\cite{bhattacharjee2020more} found users preferred less intrusive interfaces in a social dining scenario, specifically a web interface over a voice interface.
% Our work aims to close these gaps by focusing on learning when to feed a users in triadic scenarios while using features from all diners.

% \textbf{Interruption Timing Prediction}
% Researchers have found that people performed best on a task if interruptions were mediated rather than timed immediately or on scheduled intervals \cite{mcfarlane2002comparison,czerwinski2000instant} .
% As sensors become more widespread and large amounts of data is easier to collect, machine-learning based approaches are becoming more accurate at predicting interruptibility by considering contextual and social factors \cite{pielot2017beyond, takemae2007estimating, banerjee2018effects, wu2021learning}.

% Capturing natural social interactions in computational models are crucial to provide services without distracting users from the social ambiance. 
% Gaze, speaking interactions, body pose have all been effective measures in learning social signals of humans \cite{wang2021multi, muller2018robust, park20123d}.
% Joo et al.~\cite{joo2019towards} presented a framework to model social interactions by predicting whether a person is speaking or by predicting their body gestures while looking only at other conversational partners.
% Similarly, this work focuses on capturing social interactions from a set of diners to develop a bite timing strategy that can feed a target user on a robot.

% McFarlane~\cite{mcfarlane2002comparison} and Czerwinski et al.~\cite{czerwinski2000instant} found that people performed best on a primary continuous task if interruptions were mediated rather than timed immediately or on scheduled intervals.
% Using data of able-bodied humans eating together, we propose leveraging similar models on interruptibility to learn when an ideal time a robot should interrupt a user to feed.

% For example, Pielot et al.~\cite{pielot2017beyond} used a machine-learning-based approach to notify users at opportune moments based on contextual factors.
% Other research has used computer vision to determine moments to interrupt people.
% Takemae et al.~\cite{takemae2007estimating} used computer vision for activity tracking in a Japanese home with video collected over three weeks and developed a support vector regression model that had a correlation coefficient of $R^{2}=0.32$ with people's own rating of their interruptibility. 
% Takemae et al.~\cite{takemae2007estimating} developed a model for interruptibility in the home and found a slight correlation to people's own rating of their interruptibility.
% Banerjee et al.~\cite{banerjee2018effects}  developed a robot that used person and object recognition from YOLO~\cite{redmon2017yolo9000}, Microsoft's Common Objects in Context \cite{lin2014microsoft}, and Faster-RCNN~\cite{ren2015faster} to guess when participants were idle or on-task and help the robot decide when to ask for assistance. 
% Banerjee et al.~\cite{banerjee2018effects} developed a system that used social and contextual cues to estimate when a robot should interrupt a user conducting a task. They found their system interrupts at more appropriate times than a robot without interruptability awareness.
% Wu et al.~\cite{wu2021learning} developed an in-vehicle agent that used multi-sensor fusion method to predict well-timed moments to talk with drivers by sensing internal and external features.
% by sensing physiological measurements, CAN-bus data and visual features. 
% to eat by learning on a data of able-bodied humans eating


% \textbf{Social Signals Modeling}
% Capturing natural social interactions in computational models are crucial to provide services without distracting users from the social ambiance. 
% Gaze, speaking interactions, body pose have all been effective measures in learning social signals of humans \cite{wang2021multi, muller2018robust, park20123d}.
% Joo et al.~\cite{joo2019towards} presented a framework to model social interactions by predicting whether a person is speaking or by predicting their body gestures while looking only at other conversational partners.
% Similarly, this work focuses on capturing social interactions from a set of diners to develop a bite timing strategy that can feed a target user on a robot.

% \cite{wang2021multi} proposed a framework for multi-person 3D motion trajectory prediction which utilized a local-range encoder for individual motion and a global-range encoder for social interactions. 
% \cite{muller2018robust} studied how gaze contacts and speaking interactions could reveal social cues and human interactions. 
% Park et al.~\cite{park20123d} used head-mounted cameras to detect social saliency. 



